Verifiable and Provably Secure Machine Unlearning

Machine unlearning aims to remove points from the training dataset of a machine learning model after training: e.g., when a user requests their data to be deleted. While many unlearning methods have been proposed, none of them enable users to audit the procedure. Furthermore, recent work shows a user is unable to verify whether their data was unlearnt from an inspection of the model parameter alone. Rather than reasoning about parameters, we propose to view verifiable unlearning as a security problem. To this end, we present the first cryptographic definition of verifiable unlearning to formally capture the guarantees of an unlearning system. In this framework, the server first computes a proof that the model was trained on a dataset D. Given a user's data point d requested to be deleted, the server updates the model using an unlearning algorithm. It then provides a proof of the correct execution of unlearning and that d is not part of D', where D' is the new training dataset (i.e., d has been removed). Our framework is generally applicable to different unlearning techniques that we abstract as admissible functions. We instantiate a protocol in the framework, based on cryptographic assumptions, using SNARKs and hash chains. Finally, we implement the protocol for three different unlearning techniques and validate its feasibility for linear regression, logistic regression, and neural networks.

==> contents/figures/completeness.tex <==
\nicoresetlinenr
\begin{figure}[t]
	\centering
	\hspace*{-0.2cm}
	\scalebox{0.90}{
		\fbox{\small
			\begin{minipage}[t]{9.15cm}
			    \underline{$\gameCompleteness_{\advA,\protocol,\alldata}(1^\secpar)$}
			    \begin{nicodemus}
			        \item $\pub\gets\Setup(1^\secpar)$
			        \item $(\sk,\pk)\gets\AuditorSetup(1^\secpar)$
			        \item $(\stateS,\com,\model,\proofModel)\gets\Init(\pub)$
			        \item $(\state,\sigA)\gets\VrfyInit(\sk,\pub,\com,\model,\proofModel)$
			        \item $\pcif \sigA=\bot\colon$
			        \item \quad $\abort$
			        \item $\listDataAdd\coloneqq [\emptyset]$, $\listDataUnlearnAdd\coloneqq [\emptyset]$, $\listQueries\coloneqq [(\com,\sigA)]$, $\cntIteration\coloneqq 0$
			        \item $\advA^{\OracleUpdate,\OracleUnlearn}(\pub,\pk)$
			        \item \pcreturn $1$
			    \end{nicodemus}
			    \ \\
			    \underline{$\OracleUpdate(\dataAdd,\dataUnlearnAdd)$}
				\begin{nicodemus}
				    \item \pcif $\exists \dataAddP\in\listDataAdd$ s.t. $\dataAdd\cap\dataAddP\neq\emptyset~ \pcor$
				    \item[] \phantom{\pcif}$\exists \dataUnlearnAddP\in\listDataUnlearnAdd$ s.t. $\dataAdd\cap\dataUnlearnAddP\neq\emptyset\colon$
				    \item \quad ~\pcreturn $\bot$
				    \item $(\stateS,\com,\model,\proofModel,\up)\gets\ProveUpdate(\stateS,\pub,\dataAdd,\dataUnlearnAdd)$
				    \item $(\state,\sigA)\gets\VrfyUpdate(\state,\sk,\pub,\com,\model,\proofModel,\up)$
			        \item $\pcif \sigA=\bot\colon$
			        \item \quad $\abort$
			        \item $\listDataAdd.\append(\dataAdd)$, $\listDataUnlearnAdd.\append(\dataUnlearnAdd)$
			        \item $\listQueries.\append(\com,\sigA)$, $\cntIteration\coloneqq \cntIteration+1$
			        \item \pcreturn
			     \end{nicodemus}
			     \ \\
			    \underline{$\OracleUnlearn(d)$}
				\begin{nicodemus}
				    \item \pcif $d\notin\listDataUnlearnAdd[\cntIteration]\colon$
				    \item \quad \pcreturn $\bot$
				    \item $\proofUnlearn\gets\ProveUnlearn(\pub,\stateS,d)$
				    \item $(\com,\sigA)\coloneqq\listQueries[\cntIteration]$
				    \item $\pcif \pcnot \VrfyUnlearn(\pub,\pk,\cntIteration,d,\com,\sigA)\colon$
				    \item \quad \pcabort
			        \item \pcreturn
			     \end{nicodemus}
			\end{minipage}
	}}
	\caption{
		\textbf{Completeness Game.} We define the completeness of an unlearning protocol $\protocol$ in terms of game $\gameCompleteness$.
		\label{fig:completeness}}
\end{figure}

==> contents/figures/instantiated_protocol.tex <==
\begin{figure*}[t!]
\centering
\hspace*{-0.05cm}\resizebox{1.02\textwidth}{!}{
	\begin{tikzpicture}
	\matrix (m0) [matrix of math nodes,row sep=-0.3em,column sep=0em,minimum width=1em,minimum height=1em,ampersand replacement=\&,
	column 1/.style={anchor=base west},
	column 4/.style={anchor=base west},
	column 7/.style={anchor=base west}] {
~~\textbf{Users}~\users~ \{(\relationI,\relationT,\relationU),(\ppI,\ppT,\ppU),\userdata\sim\alldata\}_{\cntUser\in\users} \& \hspace*{2.8cm} \& \hspace*{2.8cm} \& ~~\textbf{Server}~\server~((\relationI,\relationT,\relationU),(\ppI,\ppT,\ppU),(\initFunction,\trainingFunction,\unlearningFunction),\seed) \& \;
\\
%
\; \& \; \& \; \& \; \& \;
\\
%
\; \& \; \& \; \& (\stF[,0],\model[0])\coloneqq\initFunction(\seed)
\& \; 
\\
%
\; \& \; \& \; \& \hashsData[0]\coloneqq \emptyset, \hashsUnlearned[0]\coloneqq \emptyset \& \; 
\\
%
\; \& \; \& \; \& \com[0]\coloneqq (\HashState(\stF[,0]),\HashModel(\model[0]),\& \;
\\
%
\; \& \; \& \; \& \phantom{\com[0]\coloneqq(}\HashData(\hashsData[0]),\HashDataUnlearn(\hashsUnlearned[0]))  \& \;
\\
%
\; \& \; \& \; \& \text{Compute } (\statement_0,\witness_0)\in\relationI \text{ using } \com[0] \text{ and } (\stF[,0],\model[0]) \& \;
\\
%
\quad \text{Verify } \statement_0 \text{ valid for } \com[0] \& \; \& \; \& \proofI[0]\gets\SNARKProve(\relationI,\ppI,\statement_0,\witness_0) \& \; 
\\
%
\quad \pcif \pcnot \SNARKVrfy(\relationI,\ppI,\proofI[0],\statement_0)\colon \& \; \& \; \& \stS[0]\coloneqq(\stF[,0],\hashsData[0],\hashsUnlearned[0],\com[0]) \& \;
\\
% 
\quad \quad \pcabort \& \; \& \; \& \dataAdd[0]\coloneqq\emptyset,~ \dataUnlearnAdd[0]\coloneqq\emptyset \& \;
\\
% 
\; \& \; \& \; \& \; \& \; 
\\
%
\; \& \; \& \; \& \; \& \; 
\\
%
\; \& \; \& \; \& \dataAdd[\cntIteration]\coloneqq\dataAdd[\cntIteration-1],~ \dataUnlearnAdd[\cntIteration]\coloneqq\dataUnlearnAdd[\cntIteration-1] \& \;
\\
%
\; \& \; \& \; \& \; \& \;
\\
%
\hspace*{0.8cm}\codecomment{add data samples} \& \; \& \; \& \; \& \;
\\
%
\hspace*{0.9cm}\cntAdd\text{-th query} \& \; \& \; \& \dataAdd[\cntIteration]\coloneqq\dataAdd[\cntIteration]\cup\{(\cntUser,d_{\cntIteration,\cntAdd})\} \& \;
\\
%
\; \& \; \& \; \& \; \& \; 
\\
%
\hspace*{0.8cm}\codecomment{remove data samples} \& \; \& \; \& \; \& \; 
\\
%
\hspace*{0.9cm}\cntDelete\text{-th query} \& \; \& \; \& \dataUnlearnAdd[\cntIteration]\coloneqq\dataUnlearnAdd[\cntIteration]\cup\{(u,d_{\cntIteration,\cntDelete})\} \& \;
\\
%
\; \& \; \& \; \& \; \& \; 
\\
%
\; \& \; \& \; \& \; \& \; 
\\
%
\; \& \; \& \; \& \text{Parse } \stS[\cntIteration-1] \text{ as } (\stF[,\cntIteration-1],\hashsData[\cntIteration-1],\hashsUnlearned[\cntIteration-1],\hStF[\cntIteration-1],\hModel[\cntIteration-1],\hData[\cntIteration-1],\hUnlearn[\cntIteration-1]) \; \& \; 
\\
%
\; \& \; \& \; \& (\stF[,\cntIteration],\model[\cntIteration])\coloneqq\trainingFunction(\stF[,\cntIteration-1],\dataAdd[\cntIteration]) \& \;
\\
%
\; \& \; \& \; \& \hashsData[\cntIteration]\coloneqq \hashsData[\cntIteration-1] \cup \{\HashDataSample(\cntUser,d)\}_{(\cntUser,d)\in\dataAdd[\cntIteration]} \& \; 
\\
%
\; \& \; \& \; \& \com[\cntIteration]\coloneqq (\HashState(\stF[,\cntIteration]),\HashModel(\model[\cntIteration]), \& \;
\\
%
\; \& \; \& \; \& \phantom{\com[\cntIteration]\coloneqq(}\HashData(\hashsData[\cntIteration]),\hUnlearn[\cntIteration-1]) \& \; 
\\
%
\; \& \; \& \; \& \text{Compute $(\statement_{\cntIteration},\witness_{\cntIteration}) \in \relationT$ using } (\hStF[,\cntIteration-1],\hData[\cntIteration-1],\hUnlearn[\cntIteration-1],\com[\cntIteration]) \& \;
\\
%
\; \& \; \& \; \& \phantom{\text{Compute  }(\statement_{\cntIteration},\witness_{\cntIteration}) \in \relationT~} \text{~ and }(\stF[\cntIteration-1],\hashsUnlearned[\cntIteration-1],\dataAdd[\cntIteration]) \& \;
\\
%
\qquad \text{Verify } \statement_\cntIteration \text{ valid for } (\com[\cntIteration-1],\com[\cntIteration])  \& \; \& \; \& \proofT[\cntIteration]\gets\SNARKProve(\relationT,\ppT,\statement_{\cntIteration},\witness_{\cntIteration})  \& \;
\\
%
\qquad \pcif \pcnot \SNARKVrfy(\relationT,\ppT,\proofT[\cntIteration],\statement_\cntIteration)\colon \& \; \& \; \& \stS[\cntIteration]\coloneqq(\stF[,\cntIteration],\hashsData[\cntIteration],\hashsUnlearned[\cntIteration],\com[\cntIteration]) \& \; 
\\
%
\qquad \quad \pcabort \& \; \& \; \& \dataAdd[\cntIteration]\coloneqq\emptyset \& \; 
\\
%
\; \& \; \& \; \& \; \& \; 
\\
%
\; \& \; \& \; \& \; \& \; 
\\
%
\; \& \; \& \; \& \text{Parse } \stS[\cntIteration-1] \text{ as } (\stF[,\cntIteration-1],\hashsData[\cntIteration-1],\hashsUnlearned[\cntIteration-1],\hStF[\cntIteration-1],\hModel[\cntIteration-1],\hData[\cntIteration-1],\hUnlearn[\cntIteration-1]) \& \; 
\\
%
\; \& \; \& \; \&  (\stF[,\cntIteration],\model[\cntIteration])\coloneqq\unlearningFunction(\stF[,\cntIteration-1],\dataUnlearnAdd[\cntIteration]) \& \;
\\
%
\; \& \; \& \; \& \hashsUnlearned[\cntIteration]\coloneqq \hashsUnlearned[\cntIteration-1] \cup \{\HashDataSample(\cntUser,d)\}_{(\cntUser,d)\in\dataUnlearnAdd[\cntIteration]} \& \;
\\
%
\; \& \; \& \; \& \hashsData[\cntIteration]\coloneqq \hashsData[\cntIteration-1] \setminus \{\HashDataSample(\cntUser,d)\}_{(\cntUser,d)\in\dataUnlearnAdd[\cntIteration]} \& \;
\\
%
\; \& \; \& \; \& \com[\cntIteration]\coloneqq (\HashState(\stF[,\cntIteration]),\HashModel(\model[\cntIteration]), \& \;
\\
%
\; \& \; \& \; \& \phantom{\com[\cntIteration]\coloneqq(}\HashData(\hashsData[\cntIteration]),\HashDataUnlearn(\hashsUnlearned[\cntIteration])) \& \; 
\\
%
\;  \& \; \& \; \& \text{Compute $(\statement_{\cntIteration},\witness_{\cntIteration}) \in \relationU$ using } (\hStF[,\cntIteration-1],\hData[\cntIteration-1],\hUnlearn[\cntIteration-1],\com[\cntIteration]) \& \;
\\
%
\; \& \; \& \; \& \phantom{\text{Compute  }(\statement_{\cntIteration},\witness_{\cntIteration}) \in \relationU~} \text{~ and }(\stF[\cntIteration-1],\hashsData[\cntIteration-1],\dataUnlearnAdd[\cntIteration]) \& \;
\\
%
\qquad \text{Verify } \statement_\cntIteration \text{ valid for } (\com[\cntIteration-1],\com[\cntIteration])  \& \; \& \; \& \proofU[\cntIteration]\gets\SNARKProve(\relationU,\ppU,\statement_{\cntIteration},\witness_{\cntIteration}) \& \;
\\
%
\qquad \pcif \pcnot \SNARKVrfy(\relationU,\ppU,\proofT[\cntIteration],\statement_\cntIteration)\colon  \& \; \& \; \& \stS[\cntIteration]\coloneqq(\stF[,\cntIteration],\hashsData[\cntIteration],\hashsUnlearned[\cntIteration],\com[\cntIteration]) \& \;
\\
%
\qquad \quad \pcabort \& \; \& \; \& \; \& \; 
\\
%
\; \& \; \& \; \&  \pcfor (\cntUser,d_{\cntIteration,\cntDelete})\in \dataUnlearnAdd[\cntIteration]\colon  \& \;
\\
%
\qquad \text{Fetch } \hUnlearn[\cntIteration] \text{ from } \com[\cntIteration]  \& \; \& \; \& \quad \proofUnlearn[\cntIteration,\cntDelete]\gets\ComputeTreePath(\dUnlearn[\cntIteration,\cntDelete],\hashsUnlearned[\cntIteration]) \& \;
\\
%
\qquad \pcif \pcnot \VrfyTreePath(\hUnlearn[\cntIteration],\dUnlearn[\cntIteration,\cntDelete],\proofUnlearn[\cntIteration,\cntDelete])\colon \& \; \& \; \& \dataUnlearnAdd[\cntIteration]\coloneqq\emptyset \& \; 
\\
%
\qquad \quad ~~\pcabort \& \; \& \; \& \; \& \; 
\\
%
	};
	\draw[dashed] ([xshift=0pt,yshift=0pt] m0-2-1.west) -- ([xshift=-15pt,yshift=0pt] m0-2-5.east) node [draw=none,pos=0.025,below=0cm,black] {\textit{Initialize}};
	%
	\draw[dashed] ([xshift=0pt,yshift=3pt] m0-12-1.west) -- ([xshift=-15pt,yshift=3pt] m0-12-5.east) node [draw=none,pos=0.045,below=0cm,black] {$\cntIteration$-\textit{th iteration}};
    %
	\draw[dashed] ([xshift=20pt,yshift=0pt] m0-21-1.west) -- ([xshift=-15pt,yshift=0pt] m0-21-5.east) node [draw=none,pos=0.058,below=0cm,black] {\textit{Proof of Training}};
    %
    \draw[dashed] ([xshift=20pt,yshift=3pt] m0-33-1.west) -- ([xshift=-15pt,yshift=3pt] m0-33-5.east) node [draw=none,pos=0.072,below=0cm,black] {\textit{OR Proof of Unlearning}};
	%
    %
    \draw[>=latex,->] ([xshift=10pt,yshift=0pt] m0-8-3.east) -- ([xshift=-10pt,yshift=0pt] m0-8-2.west) node [draw=none,midway,above=0cm,black] {$\com[0],\proofModel[0]\coloneqq(\statement_0,\proofI[0])$};
    %
	\draw[>=latex,->] ([xshift=-10pt,yshift=0pt] m0-16-2.west) -- ([xshift=10pt,yshift=0pt] m0-16-3.east) node [draw=none,midway,above=0cm,black] {$\cntUser\in\users,~\dUnlearn[\cntIteration,\cntAdd]\in\userdata$};
	%
	\draw[>=latex,->] ([xshift=-10pt,yshift=0pt] m0-19-2.west) -- ([xshift=10pt,yshift=0pt] m0-19-3.east) node [draw=none,midway,above=0cm,black] {$\cntUser\in\users,~\dUnlearn[\cntIteration,\cntDelete]\in\userdata$};
	%
	\draw[>=latex,->] ([xshift=10pt,yshift=0pt] m0-29-3.east) -- ([xshift=-10pt,yshift=0pt] m0-29-2.west) node [draw=none,midway,above=0cm,black] {$\train\com[\cntIteration],\proofModel[\cntIteration]\coloneqq(\statement_{\cntIteration},\proofT[\cntIteration])$};
	%
    \draw[>=latex,->] ([xshift=10pt,yshift=0pt] m0-42-3.east) -- ([xshift=-10pt,yshift=0pt] m0-42-2.west) node [draw=none,midway,above=0cm,black] {$\unlearn\com[\cntIteration],\proofModel[\cntIteration]\coloneqq(\statement_{\cntIteration},\proofU[\cntIteration])$};
	%
    \draw[>=latex,->] ([xshift=10pt,yshift=0pt] m0-45-3.east) -- ([xshift=-10pt,yshift=0pt] m0-45-2.west) node [draw=none,midway,above=0cm,black] {$\proofUnlearn[\cntIteration,\cntDelete]$};
    %
	%
	\draw[draw=gray] ([xshift=0pt,yshift=-1pt] m0-3-4.north west) rectangle ([xshift=83pt,yshift=2pt] m0-9-4.south east) node [draw=none,black,below=-0.05cm,anchor=north east] {\footnotesize{$\Init$}};
	%
	\draw[draw=gray] ([xshift=10pt,yshift=0pt] m0-8-1.north west) rectangle ([xshift=-60pt,yshift=0pt] m0-10-2.south west) node [draw=none,black,above=2cm,anchor=north east] {\footnotesize{$\VrfyInit$}};
    %
    \draw[draw=gray] ([xshift=0pt,yshift=-1pt] m0-22-4.north west) rectangle ([xshift=-2pt,yshift=0pt] m0-30-5.south west)node [draw=none,black,below=-0.05cm,anchor=north east] {\footnotesize{$\ProveUpdate$}};
    %
	\draw[draw=gray] ([xshift=20pt,yshift=0pt] m0-29-1.north west) rectangle ([xshift=-50pt,yshift=0pt] m0-31-2.south east) node [draw=none,black,above=2cm,anchor=north east] {\footnotesize{$\VrfyUpdate$}};
    %
	\draw[draw=gray] ([xshift=0pt,yshift=0pt] m0-34-4.north west) rectangle ([xshift=-2pt,yshift=0pt] m0-43-5.south west) node [draw=none,black,below=-0.05cm,anchor=north east] {\footnotesize{$\ProveUnlearn$}};
    %
    \draw[draw=gray] ([xshift=20pt,yshift=0pt] m0-42-1.north west) rectangle ([xshift=-50pt,yshift=1pt] m0-44-2.south east) node [draw=none,black,above=1.95cm,anchor=north east] {\footnotesize{$\VrfyPubUnlearn$}};
    %
	\draw[draw=gray] ([xshift=0pt,yshift=0pt] m0-45-4.north west) rectangle ([xshift=-10pt,yshift=0pt] m0-46-5.south east) node [draw=none,black,below=-0.05cm,anchor=north east] {\footnotesize{$\ProvePrivUnlearn$}};
    %
	\draw[draw=gray] ([xshift=20pt,yshift=0pt] m0-46-1.north west) rectangle ([xshift=-50pt,yshift=1pt] m0-48-2.south east) node [draw=none,black,above=2cm,anchor=north east] {\footnotesize{$\VrfyPrivUnlearn$}};
    %
	\coordinate (B) at (current bounding box.south west);
	\draw[line width=0.5pt]
	let
	\p2 = ($(B) - (1mm, 0mm)$)
	in
	(current bounding box.north east) ++(-4mm,1mm) rectangle (\p2);
	\end{tikzpicture}
}
        \caption{\emph{Instantiated Protocol $\protocolF$.}  We instantiate the protocol for the triple of admissible functions $\admissibleFunction=(\initFunction,\trainingFunction,\unlearningFunction)$ with two primitives: a SNARK $\SNARK$, and a hash function $\Hash$.
        }
	\label{fig:protocol}
 \vspace{-1em}
\end{figure*}


==> contents/includes/algorithm-circuit-full.tex <==
\nicoresetlinenr
\begin{figure}[t]
	\centering
	\hspace*{-0.15cm}\scalebox{0.77}{
		\fbox{\small
			\begin{minipage}[t]{10.05cm}
   				\underline{$\circuitInit(\textbf{public } \hStF[,0],\hModel[0],\hData[0],\hUnlearn[0], \textbf{ private } \stF[,0], \model[0]$)~}
				\begin{nicodemus}
                    \item \codecomment{Check input for initialization}
                    \item \pcif $\hStF[,0]\neq\HashState(\stF[,0])$ \pcor
                    \item[] \phantom{\pcif}$\hModel[0]\neq\HashModel(\model[0])$ \pcor
                    \item[] \phantom{\pcif}$\hData[0]\neq\HashData(\emptyset)$ \pcor
                    \item[] \phantom{\pcif}$\hUnlearn[0]\neq\HashDataUnlearn(\emptyset)\colon$
                    \item \quad \hspace*{0.1cm}$\pcreturn \false$
                    \item \vspace{0.3em} $\pcreturn \true$
				\end{nicodemus}
                \ \\
                \underline{$\circuitTraining(\textbf{public } \hStF[,\cntIteration],\hStF[,\cntIteration-1],\hModel[\cntIteration],\hData[\cntIteration],\hData[\cntIteration-1],\hUnlearn[\cntIteration],\hUnlearn[\cntIteration-1],$}\\
                \hspace*{0.45cm}\underline{$\textbf{ private } \stF[,\cntIteration-1],\hashsUnlearned[\cntIteration-1],\dataAdd[\cntIteration])~$}
				\begin{nicodemus}
                    \item \codecomment{Check input set of hashed unlearnt data records}
                    \item \pcif $\hUnlearn[\cntIteration-1]\neq\HashDataUnlearn(\hashsUnlearned[\cntIteration-1])\colon$
                    \item \quad \hspace*{0.1cm}$\pcreturn \false$
                    %
                    \item \vspace{0.3em}\codecomment{Update and check set of hashed training data records and unlearnt data records}
                    \item $\hashsDataAdd[\cntIteration]\coloneqq \{\HashDataSample(\cntUser,d)\}_{(\cntUser,d)\in\dataAdd[\cntIteration]}$
                    \item $\pcif \hData[\cntIteration]\neq \AppendHashData(\hData[\cntIteration-1],\hashsDataAdd[\cntIteration])$ \pcor 
                    \item[] \phantom{\pcif}$\hUnlearn[\cntIteration]\neq\hUnlearn[\cntIteration-1]$ \pcor
                    \item[] \phantom{\pcif}$\hashsUnlearned[\cntIteration-1]\cap\hashsDataAdd[\cntIteration]\neq \emptyset\colon$
                    \item \quad \hspace*{0.1cm}$\pcreturn \false$
                    \item \vspace{0.3em} \codecomment{Check input state, perform training and check outputs}
                    \item \pcif $\hStF[,\cntIteration-1]\neq\HashState(\stF[,\cntIteration-1])\colon$
                    \item \quad \pcreturn $\false$
                    \item $(\stF[,\cntIteration],\model[\cntIteration])\coloneqq\trainingFunction(\stF[,\cntIteration-1],\dataAdd[\cntIteration])$
                    \item \pcif $\hStF[,\cntIteration]\neq\HashState(\stF[,\cntIteration])$ \pcor
                    $\hModel[\cntIteration]\neq\HashModel(\model[\cntIteration])\colon$
                    \item \quad \hspace*{0.1cm}$\pcreturn \false$
                    \item \vspace{0.3em} $\pcreturn \true$
				\end{nicodemus}
                \ \\
				\underline{$\circuitUnlearning(\textbf{public } \hStF[,\cntIteration],\hStF[,\cntIteration-1],\hModel[\cntIteration],\hData[\cntIteration],\hData[\cntIteration-1],\hUnlearn[\cntIteration],\hUnlearn[\cntIteration-1],$}\\
                \hspace*{0.45cm}\underline{$\textbf{ private } \stF[,\cntIteration-1], \hashsData[\cntIteration-1],\dataUnlearnAdd[\cntIteration])$~}
				\begin{nicodemus}
                    \item \codecomment{Check input set of hashed training data records}
                    \item \pcif $\hData[\cntIteration-1]\neq\HashData(\hashsData[\cntIteration-1])\colon$
                    \item \quad \hspace*{0.1cm}$\pcreturn \false$
                    %
                    \item \vspace{0.3em}\codecomment{Update and check set of hashed unlearnt data records and training data records}
                    \item $\hashsUnlearnedAdd[\cntIteration]\coloneqq \{\HashDataSample(\cntUser,d)\}_{(\cntUser,d)\in\dataUnlearnAdd[\cntIteration]}$
                    \item $\hashsData[\cntIteration]\coloneqq\hashsData[\cntIteration-1] \setminus \hashsUnlearnedAdd[\cntIteration]$
                    \item $\pcif \hUnlearn[\cntIteration]\neq\AppendHashDataUnlearn(\hUnlearn[\cntIteration-1],\hashsUnlearnedAdd[\cntIteration])$ \pcor
                    $\hData[\cntIteration]\neq\HashData(\hashsData[\cntIteration])\colon$
                    \item \quad \hspace*{0.1cm}$\pcreturn \false$
                    %
                    \item \vspace{0.3em} \codecomment{Check input state, perform unlearning and check outputs}
                    \item $\hStF[,\cntIteration-1]\neq\HashState(\stF[,\cntIteration-1])\colon$
                    \item \quad \pcreturn $\false$
                    \item $(\stF[,\cntIteration],\model[\cntIteration])\coloneqq\unlearningFunction(\stF[,\cntIteration-1],\dataUnlearnAdd[\cntIteration])$
                    \item \pcif $\hStF[,\cntIteration]\neq\HashState(\stF[,\cntIteration])$ \pcor
                    $\hModel[\cntIteration]\neq\HashModel(\model[\cntIteration])\colon$
                    \item \quad \hspace*{0.1cm}$\pcreturn \false$
                    \item \vspace{0.3em} $\pcreturn \true$
				\end{nicodemus}
\end{minipage}}}
    % \vspace{-0.5em}
	\caption{\emph{Circuits $\circuitInit$, $\circuitTraining$ and $\circuitUnlearning$.} Based on this circuits, we prove correct execution of admissible functions for initialization, proof of training and proof of unlearning. %The hash algorithms are further specified in \cref{app:protocol}.
	\label{fig:circuits}}
 \vspace{-1em}
\end{figure}


==> contents/includes/table-datasets.tex <==
\begin{table}[t]
\centering
\caption{\emph{Scalability to Benchmark Datasets.} We compute the proof of training for different datasets from the PMLB benchmark suite~\cite{romano-21-pmlb}.}
% \vspace{-0.5em}
\label{table:datasets}
\resizebox{\columnwidth}{!}{
\begin{tabular}{@{}lccccccccc@{}}
\toprule
    \multicolumn{1}{@{}l}{ {{\bf Dataset}} }
&& \multicolumn{2}{@{}c}{ {{\bf Size}} } 
&& \multicolumn{1}{@{}c}{ {{\bf R1CS}} } 
&& \multicolumn{1}{@{}c}{ $\boldsymbol{\SNARKProve}$ }
&& \multicolumn{1}{@{}c}{ $\boldsymbol{\SNARKVrfy}$ }  \\
\midrule
\midrule
Creditscore && $100 $&$ 6$ && 3,986,308 &&  2m 22s &&  0m 47s \\
\rule{0pt}{2ex}%<--- do not remove \\
Patient &&  $88 $&$ 8$ && 4,579,718 &&  2m 28s &&  0m 53s \\
\rule{0pt}{2ex}%<--- do not remove \\
Cy Young &&  $92 $&$ 10$ && 5,903,988 &&  3m 16s &&  1m  9s \\
\rule{0pt}{2ex}%<--- do not remove \\
Corral && $160 $&$ 6$ && 6,347,236 &&  3m 43s &&  1m 15s \\
\rule{0pt}{2ex}%<--- do not remove \\
Lawsuit && $264 $&$ 4$  && 7,190,981 &&  4m  7s &&  1m 27s \\
\rule{0pt}{2ex}%<--- do not remove \\
Breast cancer && $286 $&$ 9$  && 16,514,048 &&  9m 25s &&  3m 18s \\
\rule{0pt}{2ex}%<--- do not remove \\
Monk3 && $554 $&$ 6$  && 21,841,281 && 13m 36s &&  4m 32s \\
\bottomrule
\end{tabular}}
\begin{flushleft}
\scriptsize{{Size}: \#data points $\times$ \#features}\\
\scriptsize{{R1CS}: \#constraints}\\
\end{flushleft}
\vspace{-2em}
\end{table}

